Deepfake Detection using Spatiotemporal Convolutional Networks

Better generative models and larger datasets have led to more realistic fake videos that can fool the human eye but produce temporal and spatial artifacts that deep learning approaches can detect. Most current Deepfake detection methods only use individual video frames and therefore fail to learn from temporal information. We created a benchmark of the performance of spatiotemporal convolutional methods using the Celeb-DF dataset. Our methods outperformed state-of-the-art frame-based detection methods. Code for our paper is publicly available at https://github.com/oidelima/Deepfake-Detection.

==> Intro.tex <==
In recent years, DeepFakes have become an increasing threat to social security, privacy and democracy. As a result, research in the detection of such DeepFake videos have taken many different approaches. Initial methods tried to exploit discrepancies in the fake video generation process, however more recent research has moved toward using deep learning approaches for this task. 
\par
From a larger perspective, DeepFake detection can be considered a binary classification problem to distinguish between `real' and `fake' videos. There are many architectures that have achieved remarkable results and these are mentioned in the following section. However, most of these methods rely only on 2D information and fail to leverage temporal information in the videos. An area of research that has delved deeper into using information across frames in a video is `Action-Recognition'. In this paper, we aim to apply techniques used for video classification, that take advantage of 3D data, on the DeepFake classification problem at hand. Although more computationally expensive in some cases, the additional information gained from these temporally-aware networks have proved to be more successful. For this work we have chosen the Celeb-DF (v2) dataset \cite{li2019celeb} which contains 590 real videos collected from YouTube and 5639 corresponding synthesised videos of high quality. 
